Synergies in analysing binary black hole mergers: Effect of orbital eccentricity, spin-precession, and non-quadrupole modes

A gravitational wave (GW) signal carries imprints of the properties of its source. The ability to extract source properties crucially depends on our prior knowledge of the signal morphology. Even though binary black hole (BBH) mergers are the cleanest system to model in general relativity, currently, there are no waveform models which include all physical effects. This thesis focuses on three subdominant effects: orbital eccentricity, spin-precession, and non-quadrupole or higher-order modes (HMs). We study the interplay of these effects on data analysis of GW signals, highlighting the shortcomings and emphasizing the need for more advanced waveforms. For instance, we investigate whether orbital eccentricity and spin-precession can mimic each other and thus caution the GW community towards the biases that may arise due to the neglect of eccentricity and/or spins in the waveform models. Using waveforms with full spin-precession and HMs, we extend the existing spin-induced quadrupole moment (SIQM) test - a null test to distinguish BBH systems from other black hole mimickers - and show that these improved waveforms give significantly better bounds. Additionally, we quantify the parameter space where the effect of HMs is most significant and show the importance of detecting these modes in GW events for future ground-based GW detectors such as Cosmic Explorer and Einstein Telescope.

==> 0-prematter/pre-cert-attr.tex <==
% In order to effectively convey the idea presented in this Thesis, the following work of other authors or sources was reprinted in the Thesis with their permission:
% \begin{enumerate}
% \item Figures [so and so] are distributed under the GNU GPL v2 or higher and are free to use. Figures [so and so] are distributed under the Creative Commons Attribution-Share Alike 4.0 International license and are free to use
% \item Figure [xyz] is copyright Aurelio A. Heckert, and licensed under the Free Art License. Figure [this] is freely distributed under the Artistic License v2 or higher
% \end{enumerate}
% \par


==> 0-prematter/pre-cert-guides.tex <==
\vspace{2\parskip}
\begingroup
\singlespacing
\begin{flushright}
\textbf{Dr. Chandra Kant Mishra}    \\
Research advisor        \\
Assistant Professor               \\
Department of Physics  \\
IIT Madras              \\

\par
\end{flushright}
\endgroup
\par


==> 1-frontmatter/front-abstract.tex <==
\chapter{Abstract}
\begin{tabular}{@{} >{\bfseries}p{0.2\textwidth} p{0.77\textwidth} @{}}
\MakeUppercase{Keywords} &
Gravitational waves; Binary Black holes; test of GR; eccentricity; non-quadrupole/higher modes; spin-induced quadrupole moment, spin-precession.\\
\end{tabular}
\par

\begin{doublespacing}
While the first direct detection of gravitational wave (GW) signal was from a ``vanilla'' binary black hole (BBH) system, additional physical effects have been observed in the subsequent GW signals. Even though binary black hole mergers are one of the cleanest systems to model in general relativity, currently, there are no waveform models that include all physical effects. In order to correctly characterize the source properties of a GW signal, it is imperative to understand and quantify the biases which are introduced due to missing physics in the current waveforms. In this thesis, we have focussed on three different physical effects, namely, the orbital eccentricity, spin-precession, and non-quadrupole/higher order modes (HMs). We have studied the interplay of these effects on the analysis of GW signals, highlighting the short-comings and emphasizing the need for more advanced waveforms.

Most gravitational wave events observed so far by the LIGO and Virgo detectors are consistent with mergers of binary black holes on quasi-circular orbits. However, some events, such as GW190521, are also consistent with having non-zero orbital eccentricity at detection, which can indicate that the binary formed via dynamical interactions. Active GW search pipelines employing quasi-circular waveform templates are inefficient for detecting eccentric mergers. Additionally, analysis of GW signals from eccentric BBH, with waveform models neglecting eccentricity, can lead to biases in the recovered parameters. \cite{Divyajyoti:2023rht} explores the detectability and characterisation of eccentric signals when searches and analyses rely on quasi-circular waveform models. We find that for a reference eccentric population, the fraction of events having fitting factor (FF) $<0.95$ can be up to $\approx2.2\%$ compared to $\approx0.4\%$ for the baseline population. This results in the loss in signal recovery fraction for up to $6\%$ for the region in parameter space with non-negligible eccentricity ($e_{10\,\text{Hz}} > 0.01$) and high mass ratio ($q > 3$). We also perform parameter estimation (PE) for non-spinning and aligned-spin eccentric injections of GWs from binaries of total mass $M=35$~M$_\odot$, based on numerical relativity simulations and an EOB based inspiral-merger-ringdown model (\texttt{TEOBResumS}), and recover them using both quasi-circular and eccentric waveform models. For $e_{20\,\text{Hz}}\sim 0.1$, analyses using quasi-circular waveform models are unable to recover the injected chirp mass within the $90\%$ credible interval. Further, for these low-mass injections, spin-induced precession \textit{does not} mimic eccentricity, with PE correctly ruling out high values of effective precession parameter $\chi_p$. For injections of $e_{20\,\text{Hz}}\sim 0.1$, PE conducted with an inspiral-only eccentric waveform model correctly characterises the injected signal to within $90\%$ confidence, and recovers the injected eccentricities, suggesting that such models are sufficient for characterisation of low-mass eccentric BBH. Additionally, \cite{Chattaraj:2022tay} shows that the state-of-the-art quasi-circular models including the effect of higher modes will not be adequate in extracting source properties for signals with initial eccentricities $e_{20\,\text{Hz}}$ $\gtrsim0.1$. Findings of \cite{Divyajyoti:2023rht} and \cite{Chattaraj:2022tay} form the subject matter for Chapter \ref{chap:ecc}.

Just like eccentricity, detection of a precessing spin system can be an indicator of a binary formed in a dynamical environment. Moreover, in the past few years, many of the waveform families have been upgraded to include spin-precession and higher-order modes, and are routinely used for parameter estimation and the subsequent downstream analyses, such as tests of general relativity. One of the tests which has used a precessing spin waveform model (\texttt{IMRPhenomPv2}) for the events in the third gravitational wave transient catalogue (GWTC-3) to gauge the binary black hole nature of the source \citep{LIGOScientific:2021sio}, is the spin-induced quadrupole moment (SIQM) test. In this test, bounds are obtained on a deviation parameter ($\delta{\kappa}$) related to the parameter ($\kappa$) that quantifies the degree of deformation due to the spin of individual binary components on leading (quadrupolar) spin-induced moment. In \cite{LIGOScientific:2021sio}, it was found that the spin-induced quadrupole moments of the binary black hole constituents of GWTC-3 events were consistent with those of Kerr black holes in GR. \cite{Divyajyoti:2023izl} extends the earlier SIQM-based null tests for BBH nature, by employing waveform models that account for double spin-precession and higher modes. We find that waveform with double spin-precession gives better constraints for $\delta\kappa$, compared to waveform with single spin-precession. We also revisit earlier constraints on the SIQM-deviation parameter for selected GW events observed through the first three observing runs (O1--O3) of LIGO-Virgo detectors. Additionally, the effects of HMs on the test are also explored for a variety of mass-ratio and spin combinations by injecting simulated signals in zero-noise. Our analyses indicate that binaries with mass-ratio greater than 3 and significant spin precession may require waveforms that account for spin-precession and HMs to perform the parameter estimation reliably. Results based on \cite{Divyajyoti:2023izl} and those presented in SIQM section of \cite{LIGOScientific:2021sio} are included in Chapter \ref{chap:siqm}.

The relative contribution from HMs becomes significant for binaries with asymmetric masses and/or whose orbital planes are not optimally inclined towards the line of sight. \cite{Divyajyoti:2021uty} explores the detection of HMs in third-generation ground-based detectors such as Cosmic Explorer and Einstein Telescope. Using the astrophysical population of binary black holes based on events reported in the second gravitational wave transient catalog by LIGO and Virgo (GWTC-2), in conjunction with the  Madau-Dickinson model for redshift evolution of the binary black hole mergers, we assess the detectability of these HMs using a network consisting of three third-generation detectors. We find that the two sub-leading modes [(3,3) and (4,4)] can be detected in approximately 30\% of the population with a network signal-to-noise ratio of 3 or more, and for nearly 10\% of the sources, the five leading modes will be detectable. Besides, a study concerning the effect of binary's mass ratio and its orbital inclination with the observer's line-of-sight in detecting various modes is presented. For a few selected events of the LIGO-Virgo catalog, we identify the modes that would have been detected if a third-generation detector was operational when these events were recorded. We also compute the detectability of HMs by Voyager and find that only $\sim 6\%$ and $2\%$ of the detectable population will have an associated detection of (3,3) and (4,4) modes, respectively. Observing these HMs in the 3G era would have a huge impact on the science possible with these detectors, ranging from astrophysics and cosmology to testing strong-field gravity. The findings of \cite{Divyajyoti:2021uty} are included in Chapter \ref{chap-hm} of the thesis.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The GW events detected by the LIGO-Virgo detectors are consistent with GW emission from inspiralling BBHs on quasi-circular orbits. But several events have been argued to be more consistent with coming from binaries with non-negligible orbital eccentricity at detection. In our work \cite{Divyajyoti:2023rht}, we synthesize a population of eccentric binary black hole signals and calculate the loss in searches when a quasi-circular template bank is used for recovery. We find maximum loss in the parameter region with non-negligible eccentricity ($e>0.01$) and high mass ratio ($q>3$). Further, we perform parameter estimation studies \cite{Chattaraj:2022tay, Divyajyoti:2023rht} where we inject simulated binary signals with low-moderate eccentricities ($e \sim 0.1$) and show that non-spinning and aligned-spin eccentric signals when analyzed with quasi-circular templates incur biases in the chirp mass parameter such that the injected value lies outside the 90\% credible interval. Moreover, for non-spinning and aligned-spin, eccentric binaries with long inspirals (total mass $\sim 35~M_\odot$), the quasi-circular waveforms with spin-precession correctly exclude the high values of spin precession parameter ($\chi_p$) resulting in no spurious detection of spin-precession. A direct consequence of this is that a non-spinning low-mass eccentric system if analyzed using quasi-circular waveform models only, may be mistaken for a binary that formed in isolation since the quasi-circular waveform models do not enable measurements of eccentricity and the spin posteriors show no additional signatures of dynamical formation. This may lead to miscategorization of such systems as uninteresting binaries which may not be followed up with further investigations. We also showed that an inspiral-only eccentric waveform is able to recover the injected chirp mass within the 90\% confidence interval.

%Just like eccentricity, detection of a precessing spin system can be an indicator of a binary formed in dynamical environment. Moreover, in the past few years, many of the waveform families have been upgraded to include spin-precession and higher-order modes, and are routinely used for parameter estimation and the subsequent downstream analyses, such as tests of general relativity. One of the tests which has used a precessing spin waveform (\texttt{IMRPhenomPv2}) for the events in the second and third gravitational wave transient catalogues (GWTC-2 and GWTC-3) to gauge the binary black hole nature of the source \cite{LIGOScientific:2020tif, LIGOScientific:2021sio}, is the spin-induced quadrupole moment (SIQM) test. Following the prescription in Krishnendu \textit{et al.} \cite{Krishnendu:2017shb}, a deviation parameter, $\delta\kappa_s$, can be introduced in the phasing of the gravitational waveform model, such that $\kappa = 1 + \delta\kappa_s$. This then poses as a null test for binary black hole nature of the GW source. In our work \cite{Divyajyoti:2023izl}, we extend the existing SIQM test for the double precessing waveforms of the \texttt{IMRPhenomX} family and categorically investigate the effects of double spin-precession and higher modes on the bounds of $\delta\kappa_s$. Our studies show that higher mode precessing waveforms such as \texttt{IMRPhenomXPHM} may be preferred for analysis of events with mass asymmetry and non-negligible spins.

%The relative contribution from HMs becomes significant for binaries with asymmetric masses and/or whose orbital planes are not optimally inclined towards the line of sight. In \cite{Singh:2022tlh}, we show that including these in gravitational waveforms can improve the GW early warning (pre-merger detection and localization) of neutron star - black hole mergers. In a separate work \cite{Divyajyoti:2021uty}, we quantify the parameter space containing mass ratio and inclination angle to show the regions in which different HMs contribute the maximum towards the signal-to-noise ratio (SNR) of a GW signal in 3\textsuperscript{rd} generation (3G) detectors. We also explore the detectability of HMs for an astrophysically motivated population of binaries in the 3G era and show the improvement in detectability of these modes compared to the current detector networks.
\end{doublespacing}


==> 1-frontmatter/front-acknowledgements.tex <==
\chapter{Acknowledgements}

\begin{itemize}
    \item I feel great pleasure in writing that \textbf{Chandra Kant Mishra} was my thesis advisor. He guided me each and every step of the way, starting with my final year of B.Tech. followed by Ph.D. Looking at his interactions with other academics, I learned how to articulate words clearly yet with humility. He introduced me to various collaborators and always encouraged me to ask questions, however elementary. Time and again, he reminded me that I should not hesitate to disagree with him. He would listen to me patiently without dismissing my ideas or disagreements, and discuss my projects at length from different perspectives. I would never be able to thank him enough for everything that he has taught me.
    
    \item In addition to being in my Doctoral Committee (DC), \textbf{K. G. Arun} was like a co-guide to me throughout my Ph.D. Whenever I got lost in the technicalities of the projects, he always reminded me to take a step back and look at the big picture. Writing papers with him helped improve my scientific writing, and I learned various aspects of gravitational waves while attending his course. I will always be grateful to him for his encouragement and support.
    
    \item It was a great experience to collaborate with \textbf{Prayush Kumar} on \textit{ESIGMA} project. During my conversations with him, on telecons and visits to ICTS, he taught me a great deal about Gravitational Wave data analysis, and countless programming tips and tricks. He inspires me to be a better programmer and scientist, and I look forward to working with him in the future.
    
    \item I thank \textbf{B. S. Sathyaprakash} and \textbf{Anuradha Gupta} for including me in the weekly Penn State telecons. Participating in the discussions with their groups gave me an insight into various aspects of gravitational physics with the next-generation detectors. I want to thank Sathya for inviting me to visit the Penn State University and for being a wonderful host.
    
    \item I would like to thank \textbf{L. Sriramkumar} for organising various GR and Cosmology seminars. Attending these seminars provided me with broad exposure to the field. I also thoroughly enjoyed his course on Quantum Mechanics II.
    
    \item I would like to thank \textbf{Dawood Kothawala} for his intuitive questions and comments during my DC meetings and other presentations. He helped me look at topics with a different perspective and inspired me to look deeper into the results.
    
    \item I am grateful to \textbf{Suresh Govindarajan} for his encouraging words as my DC chair in various review meetings and progress reports. I also thank  \textbf{Sunethra Ramanan} for her insightful suggestions at the DC meetings.

    \item It was a pleasure to collaborate with \textbf{N. V. Krishnendu} and \textbf{Sayantani Datta} on \textit{SIQM} projects. Krishnendu guided me at every step and was always happy to help when I felt overwhelmed. Talking to Sayantani helped me keep my sanity when we were trying to meet the deadlines.

    \item I thank \textbf{Sumit Kumar}, \textbf{Aditya Vijaykumar}, and \textbf{Muhammed Saleem}, who played a major role in teaching me the subtleties of Bayesian inference pipelines and post-processing methods. Having them as collaborators on various projects was an absolute delight, and I look forward to working with them in the future.

    \item I would like to thank \textbf{Bala R. Iyer}, \textbf{Archana Pai}, and \textbf{Sukanta Bose} for guiding me from time to time on the rules and regulations of being a member of the LVK collaboration, and the members of the LIGO India Scientific Collaboration (LISC) for weekly meetings and discussions.
    
    \item I thank \textbf{Parameswaran Ajith} for the useful discussions I had while attending the group meetings at ICTS, and whenever I had a chance to meet him. It was a pleasure to collaborate with him along with \textbf{Shasvath J. Kapadia}, \textbf{Md Arif Shaikh}, and \textbf{Mukesh Kumar Singh} on the \textit{early warning} project.
    
    \item I am thankful to \textbf{Gregory Ashton} for guiding me through GW event analyses. It was a delight to meet him in Cardiff and discuss various aspects of GW data analysis.

    \item I thank \textbf{Michalis Agathos} for inviting me to visit the University of Cambridge and for the useful discussions on \textit{Test of GR} project. I also want to thank him and \textbf{Nathan Johnson-McDaniel}, for guiding me from time to time as TGR working group chairs.

    \item I thank \textbf{Isobel M. Romero-Shaw} for making my visit at Cambridge a pleasant stay. It was a pleasure to work with her on the \textit{eccentricity} project, and I look forward to our collaboration in the future.

    \item I would like to thank \textbf{Stephen Fairhurst}, \textbf{Mark Hannam}, \textbf{Geraint Pratten}, and \textbf{Thomas Dent} for discussions on various aspects of GW science during my visits to the UK and the US.

    \item I thank ICTS for organizing gravitational wave summer schools. It was a pleasure to meet and discuss various topics on GW science with \textbf{Harald Pfeiffer} and \textbf{Geoffrey Lovelace} during the summer school.

    \item I thank \textbf{Nils Andersson} for inviting me to attend the \textit{Masterclasses in Fluid Dynamics} at the University of Southampton, and for providing me with a signed copy of his book "A Gentle Wizard".

    \item I would like to thank Rahul Kashyap, Gayathri Raman, Pradeepkumar Yadav, and Lorenzo Gavassino for the wonderful time I spent in Southampton.

    \item I am thankful to Marta Colleoni, Sebastian Khan, Ajit Mehta, Ssohrab Borhanian, Collin Capano, Guillaume Faye, Patricia Schmidt, Alexandar H. Nitz, Rahul Dhurkunde, Pankaj Saini, Sajad A. Bhat, Archisman Ghosh, and Ish Gupta for their help in various projects.

    \item It was a pleasure to collaborate with Preet Baxi, Abhishek Chattaraj, Tamal RoyChowdhury, Snehal Tibrewal, Gayathri V, Sijil Jose, Kaushik Paul, and Anshu Gupta on various projects.

    \item I thank GWECS and LAAC council members for organizing various events for early career researchers, which provided me with multiple opportunities to interact with the LVK members.

    \item I would like to thank NIT Agartala for signing an MOU with IIT Madras which gave me the opportunity to transfer to IIT Madras in my final year of B.Tech. and started my journey in gravitational waves.

    \item Some of the work included in this thesis has made use of data or software obtained from the Gravitational Wave Open Science Center (GWOSC), a service of the LIGO Scientific Collaboration, the Virgo Collaboration, and KAGRA. This material is based upon work supported by NSF’s LIGO Laboratory which is a major facility fully funded by the National Science Foundation, USA. I also acknowledge the Science and Technology Facilities Council (STFC) of the United Kingdom, the Max-Planck-Society (MPS), and the State of Niedersachsen/Germany for support of the construction of Advanced LIGO and construction and operation of the GEO600 detector. Additional support for Advanced LIGO was provided by the Australian Research Council. Virgo is funded, through the European Gravitational Observatory (EGO), by the French Centre National de Recherche Scientifique (CNRS), the Italian Istituto Nazionale di Fisica Nucleare (INFN) and the Dutch Nikhef, with contributions by institutions from Belgium, Germany, Greece, Hungary, Ireland, Japan, Monaco, Poland, Portugal, Spain. KAGRA is supported by Ministry of Education, Culture, Sports, Science and Technology (MEXT), Japan Society for the Promotion of Science (JSPS) in Japan; National Research Foundation (NRF) and Ministry of Science and ICT (MSIT) in Korea; Academia Sinica (AS) and National Science and Technology Council (NSTC) in Taiwan.
    
    \item I would like to acknowledge the following computing resources: LIGO lab clusters CIT, LHO, LLO (NSF Grant Nos.~PHY-0757058 and PHY-0823459), Sarathi cluster at IUCAA, AQUA cluster and Powehi workstation at IIT Madras, Alice and SONIC clusters at ICTS-TIFR, and ATLAS cluster at AEI Hannover.

    \item I would like to thank the Science Engineering Research Board (SERB), DST, Govt. of India (SERB Grant No.~ITS/2022/001695) for funding my travel to Cardiff University to present my work in LVK conference. I would also like to acknowledge the support of SERB’s Core Research Grant No. CRG/2022/007959 for supporting part of the work presented in this thesis.

    \item I thank the Centre for Strings, Gravitation, and Cosmology, Department of Physics, IIT Madras, and University of Cambridge  for funding my academic visit to Kavli Institute of Cosmology, Cambridge.

    \item I would like to thank Newton-Bhabha/STFC funded collaboration between UK and LIGO-India, and IIT Madras Alumni fund for sponsoring my visit to University of Southampton.
    
    \item I would like to thank the developers of the following software and packages which made my life easy and saved a lot of my time: \texttt{LALSuite}, \texttt{bilby}, \texttt{bilby\_pipe}, \texttt{PyCBC}, \textsc{Mathematica}, \texttt{gwbench}, \texttt{pesummary}, \texttt{corner}, \texttt{matplotlib}, \texttt{seaborn}, \texttt{pickle}, \texttt{h5py}, \texttt{deepdish}, \texttt{pandas}, \texttt{numpy}, \texttt{scipy}, \texttt{gwpy}, \texttt{dynesty}, TeXMaker, Overleaf, Jupyter, Spyder, VS code.

    Finally I would like to acknowledge the love and support of my friends and family:
    
    \item I would like to thank all the members of GW group at IIT Madras for the interesting discussions and fun outings that we had. In particular I would like to thank Soham, Nidhi, Sweta, Rimo, Pranav, Sijil, Chinmay, Aravind, Omkar, Pratul, Shashank, Dipthi, and Diksha.

    \item I would like to thank my friends at IITM: Santosh, Sourin, and Subhojit for their friendship.
    
    \item My years at IIT Madras were made pleasant in the company of Kaushik, Abhishek, and Laxman. I look back at our humorous discussions and outings, and I cannot imagine my life at IITM without them. It feels highly formal to say that I thank them for their love and care.
    
    \item I thank Uddeepta, Souvik, and Anup for all the fun I had whenever I visited ICTS, and for making me feel part of their family with Mukesh. I especially thank Uddeepta for planning all our excursions in and around Bengaluru. I also thank Srashti for guiding me from time to time as a loving senior whenever I was at ICTS.
    
    \item I thank Poulami, Pankaj, Parthapratim, and Sayantani for interesting discussions during our joint group meetings with the Chennai Mathematical Institute, and for always making me feel welcome when I visited their campus.

    \item I thank my B.Tech. friends from NIT Agartala Siddarth, Shashank, Pushplata, and Simran for their love and care.

    \item I would like to thank Adithyan, Bhavesh, Ashwin, and Rachana for making my final year of B.Tech. at IIT Madras pleasant.

    \item I am grateful to Sahaj Marg system (Heartfulness Meditation) for being an integral part of my life and shaping me into what I am today.

    \item I want to thank my family for the part they played in my Ph.D. -- my father, Dr.~Vikas Saxena, for sparking my interest in astronomy from childhood; my mother, Manisha Saxena, for reminding me to look at life in a simple manner whenever I over-complicated things; my sisters, Purnima and Lakshmi, who were always ready for a video call whenever I needed to de-stress; and my grandmother, Chandra Lekha Saxena, for celebrating the tiniest of my achievements with love and blessings. I also thank my in-laws for their love and care.

    \item Joining directly after B.Tech., Ph.D. coursework was the most stressful part of my life. I would not have reached this stage if it wasn't for Mukesh, to whom this thesis is dedicated. He spent countless hours helping me bridge the gaps in my understanding of physics, and I learned innumerable things from him during my Ph.D. It is an honor and joy to call myself his wife.
    
\end{itemize}

==> 1-frontmatter/front-notation.tex <==
\nomenclature{$c$}{Speed of light in vacuum \hfill $\rm{m~s^{-1}}$}

\nomenclature{$G$}{Universal gravitational constant \hfill $\rm{kg^{-1} m^3 s^{-2}}$}

\nomenclature{$m_1$}{Mass of the primary (heavier) object in the binary \hfill \Msun}

\nomenclature{$m_2$}{Mass of the secondary (lighter) object in the binary \hfill \Msun}

\nomenclature{$m_i^\text{source}$}{Source-frame mass of the $i$\textsuperscript{th} object $m_i^\text{source} = m_i/(1+z)$ \hfill \Msun}

\nomenclature{$\mathcal{M}$}{Chirp mass of the binary $\mathcal{M} = (m_1 m_2)^{3/5}/(m_1+m_2)^{1/5}$ \hfill \Msun}

\nomenclature{$M$}{Total mass of the binary $M=m_1+m_2$ \hfill \Msun}

\nomenclature{$q$}{Mass ratio $q=m_1/m_2 \geq 1$ \hfill --\,\,}

\nomenclature{$\eta$}{Symmetric mass ratio: A definition of mass ratio which is \\independent of the identity of the primary/secondary mass \\$\eta = q/(1+q)^2 \leq 0.25$ \hfill --\,\,}

\nomenclature{$\Vec{S}_i$}{Spin angular momentum vector of the $i$\textsuperscript{th} object \hfill --\,\,}

\nomenclature{$\Hat{L}$}{Unit vector along the orbital angular momentum axis of the binary \hfill --\,\,}

\nomenclature{$a_i$}{Dimensionless spin magnitude of the $i$\textsuperscript{th} object (defined at a \\reference frequency) $a_i = c \vert \Vec{S}_i\vert/(G m_i^2)$ \hfill --\,\,}

\nomenclature{$\theta_i$}{Zenith angle between the spin and orbital angular momenta for \\the $i$\textsuperscript{th} object (defined at a reference frequency) \hfill rad}

\nomenclature{$\phi_\text{JL}$}{Difference between total and orbital angular momentum azimuthal \\angles (defined at a reference frequency) \hfill rad}

\nomenclature{$\phi_{12}$}{Difference between the azimuthal angles of the individual spin vector \\projections onto the orbital plane (defined at a reference frequency) \hfill rad}

\nomenclature{$\chi_i$}{Aligned spin of $i$\textsuperscript{th} object: projection of the $i$\textsuperscript{th} object spin onto the \\orbital angular momentum (defined at a reference frequency) \\$\chi_i = a_i\cos(\theta_i)$ \hfill --\,\,}

\nomenclature{$\chi_i^\perp$}{$i$\textsuperscript{th} object in-plane spin: magnitude of the projection of the $i$\textsuperscript{th} object \\spin onto the orbital plane (defined at a reference frequency) \\$\chi_i^\perp = \vert a_i \sin(\theta_i)\vert$ \hfill --\,\,}

\nomenclature{$\chi_\text{eff}$}{Effective inspiral spin parameter $\chi_\text{eff} = (\chi_1 m_1 + \chi_2 m_2)/(m_1+m_2)$ \hfill --\,\,}

\nomenclature{$\rm{\chi_p}$}{Effective spin-precession parameter (defined at a reference \\frequency) $\rm{\chi_p} = \text{max}\{\chi_1^\perp, \chi_2^\perp q(3+4q)/(4+3q)\}$ \hfill --\,\,}

\nomenclature{$e_\text{fref}$}{Orbital eccentricity defined at a reference frequency $\rm{f_{ref}}$ \\E.g. $e_{20}$ is eccentricity defined at 20 Hz \hfill --\,\,}

\nomenclature{$\alpha$}{Right ascension \hfill rad}

\nomenclature{$\delta$}{Declination \hfill rad}

\nomenclature{$\psi$}{Polarization angle of the source \hfill rad}

\nomenclature{$\phi_c$}{Phase of coalescence of the binary \hfill rad}

\nomenclature{$d_L$}{Luminosity distance to the source \hfill Mpc}

\nomenclature{$z$}{Redshift of the source depending on specified cosmology \hfill --\,\,}

\nomenclature{$t_\text{gps}$}{GPS reference time at the geocenter \hfill s}

\nomenclature{$t_c$}{Time of coalescence of the binary \hfill s}

\nomenclature{$\iota$}{Inclination angle: Zenith angle between the orbital angular \\momentum and the line of sight \hfill rad}

\nomenclature{$\theta_\text{JN}$}{Zenith angle between the total angular momentum and the line of \\sight \hfill rad}

\nomenclature{$\kappa_i$}{SIQM parameter of the $i$\textsuperscript{th} object \hfill --\,\,}

\nomenclature{$\delta\kappa_i$}{SIQM deviation parameter of the $i$\textsuperscript{th} object $\kappa_i = 1 + \delta\kappa_i$ \hfill --\,\,}

\nomenclature{$\kappa_s$}{Symmetric combination of SIQM parameter $\kappa_s = (\kappa_1 + \kappa_2)/2$ \hfill --\,\,}

\nomenclature{$\kappa_a$}{Anti-symmetric combination of SIQM parameter $\kappa_a = (\kappa_1 - \kappa_2)/2$ \hfill --\,\,}

\nomenclature{$\delta\kappa_s$}{Symmetric combination of SIQM deviation parameter \\$\delta\kappa_s = (\delta\kappa_1 + \delta\kappa_2)/2$ \hfill --\,\,}

\nomenclature{$\delta\kappa_a$}{Anti-symmetric combination of SIQM deviation parameter \\$\delta\kappa_a = (\delta\kappa_1 - \delta\kappa_2)/2$ \hfill --\,\,}

\nomenclature{$R_{\alpha\beta}$}{Ricci tensor \hfill $\rm{m^{-2}}$}

\nomenclature{$R$}{Ricci scalar \hfill $\rm{m^{-2}}$}

\nomenclature{$g_{\alpha\beta}$}{Metric tensor \hfill --\,\,}

\nomenclature{$T_{\alpha\beta}$}{Stress-energy tensor \hfill $\rm{kg~m^{-1} s^{-2}}$}

\nomenclature{$\eta_{\alpha\beta}$}{Minkowski metric tensor \hfill --\,\,}

%\nomenclature{$R_{\alpha\beta\gamma\delta}$}{Reimann tensor \hfill $\rm{m^{-2}}$}

%\nomenclature{$G_{\alpha\beta}$}{Einstein tensor \hfill $\rm{m^{-2}}$}

\nomenclature{$p_\text{astro}$}{Probability of astrophysical origin \hfill --\,\,}

\nomenclature{$h_+$}{Plus polarization of gravitational wave strain \hfill --\,\,}

\nomenclature{$h_\times$}{Cross polarization of gravitational wave strain \hfill --\,\,}

\nomenclature{$\Msun$}{Solar mass \hfill kg}

\nomenclature{$\nu$}{PN symmetry coefficient $\nu = \vert m_1 - m_2\vert/(m_1 + m_2)$ \hfill --\,\,}

==> 2-mainmatter/chapters/extra-material-from-papers.tex <==
%HM paper

Since the discovery of the first gravitational wave (GW) event\,\cite{Abbott:2016blz} in 2015, Laser Interferometer Gravitational Wave Observatory (LIGO) Scientific Collaboration and Virgo collaboration have reported the detection of a total of 47 compact binary mergers with false alarm rate $<1\text{yr}^{-1}$\,\cite{LIGOScientific:2020ibl}. These include 44 binary black hole (BBH), two binary neutron star, and one possible neutron star-black hole (NS-BH) mergers. Additionally, independent analyses using the publicly available data\,\cite{LSC:GWTC-2-GWOSC} have confirmed these detections and have also added a few marginal BBH events to the LIGO-Virgo catalog\,\cite{Antelis:2018smo, Venumadhav:2019tad,Venumadhav:2019lyq,Nitz:2018imz,Nitz:2019hdf}. These observations have provided us with several new insights into astrophysics, cosmology, and fundamental physics (see for instance, Refs.\,\citep{TheLIGOScientific:2016htt, GBM:2017lvd, Abbott:2017xzu, LIGOScientific:2020tif, LIGOScientific:2020kqk}).

The two advanced LIGO (aLIGO) detectors \citep{LIGOScientific:2014pky} in the U.S. and advanced Virgo \citep{Acernese:2015gua} in Europe participated in the first two observing runs (named, O1 and O2), as well as for the first half of the third observation run (O3a). The Japanese detector KAGRA \citep{Akutsu:2020his} joined the LIGO-Virgo network briefly towards the end of the third observing run. The second part of the third observing run (O3b) was concluded in March 2020. 

While existing detectors are being upgraded towards LIGO A+ design \citep{Shoemaker:2019bqt, McClelland:T1500290-v3}, beyond A+ upgrades (LIGO Voyager \citep{McClelland:T1500290-v3}) and the next-generation detector configurations \cite{Punturo:2010zz, Dwyer:2014fpa} have already been proposed and science studies are currently ongoing. Cosmic Explorer (CE) \citep{McClelland:T1500290-v3, Dwyer:2014fpa, LIGOScientific:2016wof} and Einstein Telescope (ET) \cite{Punturo:2010zz, Hild:2010id} are two leading third-generation (3G) detector proposals. Both are expected to have a strain sensitivity that is an order of magnitude better than the second-generation (2G) detectors such as aLIGO and aVirgo, and a low-frequency cutoff in the range of {$1$-$5$\,Hz \cite{Chamberlain:2017fjl}}.

While BBH mergers are already the most frequently detected GW events \cite{LIGOScientific:2020ibl}, they are also among the strongest emitters of GWs and are possibly the cleanest\footnote{Near-monochromatic GW signals from isolated neutron stars too can be modeled very accurately in GR and with relative ease.} ones to model using analytical and numerical techniques in general relativity (GR) \cite{Th300}. If the gravitational waveforms are known precisely, one can use a well-known data-analysis technique called {\it matched filtering} \citep{Helstrom68} to extract signals from noisy detector output. 
The method involves cross-correlating the detector data with an accurate set of templates that closely mimic the form of expected signals and are computed in advance. The success of the method critically depends on how accurate these model predictions are. This requirement has driven the signal-modeling efforts over the past four decades by the gravitational wave community across the globe \cite{Blanchet:2013haa, Bishop:2016lgv, Sasaki:2003xr,Ajith:2007qp,Buonanno:2000ef, Poisson:2011nh, Foffa:2013qca}. 

The exact form of the GW signal depends on several intrinsic and extrinsic source parameters. Hence it is important that its theoretical predictions (templates) include all possible effects, neglect of which can potentially induce systematic biases in the measurement of source parameters or worse can even lead to non-detection of these signals. 

==> 3-backmatter/back-committee.tex <==
\chapter{\asserttoken{dissertationCommitteeName}{Committee}}
\vspace{\parskip}
\begingroup
\renewcommand*{\arraystretch}{1.25}
\begin{tabular}{@{} >{\bfseries}p{0.3\textwidth} l @{}}
    Chairperson &
        \begin{CMTsubtab}
            Prof. Suresh Govindarajan \\
            Professor  \\
            Department of Physics, Indian Institute of Technology Madras, Chennai, India - 600036.  \\
        \end{CMTsubtab} \\
    \addlinespace[0.1\textheight]
    Guide(s) &
        \begin{CMTsubtab}
            Dr. Chandra Kant Mishra  \\
            Assistant Professor  \\
            Department of Physics, Indian Institute of Technology Madras, Chennai, India - 600036.  \\
        \end{CMTsubtab} \\
    \addlinespace[0.1\textheight]
    Member(s) &
        \begin{CMTsubtab}
            Dr. Dawood Kothawala  \\
            Associate Professor  \\
            Department of Physics, Indian Institute of Technology Madras, Chennai, India - 600036.  \\
        \end{CMTsubtab} \\
        \addlinespace[4ex]
                &
        \begin{CMTsubtab}
            Prof. K. G. Arun  \\
            Professor  \\
            Chennai Mathematical Institute, H1, SIPCOT IT Park, Siruseri, Kelambakkam, India - 603103. \\
        \end{CMTsubtab} \\
        \addlinespace[4ex]
                &
        \begin{CMTsubtab}
            Dr. Sunethra Ramanan  \\
            Associate Professor  \\
            Department of Physics, Indian Institute of Technology Madras, Chennai, India - 600036. \\
        \end{CMTsubtab} \\
\end{tabular}
\endgroup


==> 3-backmatter/back-cv-education.tex <==
\CVYearAndDegree{2019}{Bachelor of Technology}
\begin{CVsubtab}
    & Institution    & National Institute of Technology \\ & & Agartala \\
    & Specialization & Engineering Physics \\
\end{CVsubtab}

\CVYearAndDegree{\the\dissertationDegree}{}
\begin{CVsubtab}
    & Institution       & Indian Institute of Technology Madras \\
    & Specialization    & Physics \\
    & Registration Date & 25 July, 2019 \\
\end{CVsubtab}


==> bibliography.tex <==
% Bibliography

\begin{singlespace}
\nocite{apsrev41Control}
%\bibliographystyle{apsrev4-1}\setstretch{0.5}
\bibliographystyle{apsrmp4-2-modified}
\bibliography{mycontrol, master}
%\bibliographystyle{iitm}
%\bibliography{master}
\end{singlespace}

==> extra_PE_parameters.tex <==
There also exist other parameters which can be inferred from the source parameters. Here, we list a few parameter combinations and inferred parameters often used in GW data analyses. First we look at the mass combinations. These include:

\begin{itemize}
    \item \textbf{chirp mass:} $\mathcal{M} = (m_1 m_2)^{3/5}/(m_1+m_2)^{1/5}$ \citep{Poisson:1995ef, Finn:1992xs, Blanchet:1995ez}
    \item \textbf{mass ratio:} $q=m_1/m_2 \geq 1$
    \item \textbf{total mass:} $M=m_1+m_2$
    \item \textbf{symmetric mass ratio:} $\eta=m_1 m_2/(m_1+m_2)^2$
    \item \textbf{eccentric chirp mass:} \citep{Favata:2021vhw} 
    \begin{equation}
        \mathcal{M}^\text{ecc} = \frac{\mathcal{M}}{(1 - \frac{157}{24}e^2)^{3/5}}
    \end{equation}
\end{itemize}

Next, we discuss spins. In addition to representing the spin vector components in cartesian coordinates, there are other representations of spins of the binary. Here, we list the representations used by \texttt{bilby\_pipe} \citep{Romero-Shaw:2020owr} which we have used extensively for data analysis in this thesis. For the rest of the parameters specified in this section we follow the notation where the subscript $i={1,2}$ indicates the primary (1) or secondary (2) object in the binary, with the assumption that the primary is the heavier of the two objects.

\begin{itemize}
    \item $\bm{a_i:}$ Dimensionless spin magnitude of the $i$\textsuperscript{th} object.
    \item $\bm{\theta_i:}$ Zenith angle between the spin and orbital angular momenta for the $i$\textsuperscript{th} object.
    \item $\bm{\phi_{12}:}$ Difference between the azimuthal angles of the individual spin vector projections onto the orbital plane.
\end{itemize}

These spin parameters can then be combined to get various other combinations:

\begin{itemize}
    \item $\bm{\chi_i:}$ Projection of the $i$\textsuperscript{th} object spin onto the orbital angular momentum\\
    $\chi_i = a_i \cos(\theta_i)$.
    \item $\bm{\chi_i^\perp:}$ Magnitude of the projection of the $i$\textsuperscript{th} object spin onto the orbital plane $\chi_i^\perp = |a_i \sin(\theta_i)|$.
    \item \textbf{$\bm{\chi_\text{eff}:}$} Effective inspiral spin parameter $\chi_\text{eff} = (\chi_1 + q \chi_2)/(1+q)$ \citep{Santamaria:2010yb, Ajith:2009bn}.
    \item \textbf{$\bm{\chi_\text{p}:}$} Effective precession spin parameter \citep{Hannam:2013oca, Schmidt:2014iyl}
    \begin{equation}
        \chi_\text{p} = \text{max}\Bigg\{ \chi_1^\perp, \frac{\chi_2^\perp}{q} \Bigg( \frac{3+4q}{4+3q} \Bigg) \Bigg\}.
    \end{equation}
\end{itemize}

It is important to note that as the binary system emits gravitational waves, the spins of the system also evolve. Thus, the spin parameters are generally measured at a reference frequency. This also holds true for other parameters such as eccentricity, binary phase, and inclination angle. A system with misaligned spin vectors w.r.t the orbital angular momentum vector undergoes spin-induced orbital precession. Thus, it is also useful to define various angles that involve the orbital angular momentum vector of the binary system:

\begin{itemize}
    \item $\bm{\iota:}$ Zenith angle between the orbital angular momentum ($\Vec{L}$) and the line of sight ($\Hat{N}$), also known as inclination angle.
    \item \textbf{$\bm{\theta_\text{JN}:}$} Zenith angle between the total angular momentum ($\Vec{J}$) and the line of sight ($\Hat{N}$).
    \item \textbf{$\bm{\phi_\text{JL}:}$} Difference between total and orbital angular momentum azimuthal angles.
\end{itemize}

We discuss spin-induced orbital precession in detail in Sec.~\ref{sec:intro-spins}. Finally, we list a few additional parameters which denote time, distance measurements, and source frame masses (which are different from the masses inferred from the gravitational wave signals in the detectors due to the redshifting of the gravitational waves).

\begin{itemize}
    \item \textbf{$\bm{t_\text{gps}:}$} GPS reference time at the geocenter, typically merger time ($t_c$).
    \item $\bm{z:}$ Redshift depending on specified cosmology.
    \item $\bm{d_C:}$ Comoving distance depending on specified cosmology.
    \item \textbf{$\bm{m_i^\text{source}:}$} Source-frame mass of the $i$\textsuperscript{th} object $m_i^\text{source} = m_i/(1+z)$ \citep{Krolak:1987ofj}.
    \item \textbf{$\bm{\mathcal{M}^\text{source}:}$} Source-frame chirp mass $\mathcal{M}^\text{source} = \mathcal{M}/(1+z)$.
    \item \textbf{$\bm{M^\text{source}:}$} Source-frame total mass $M^\text{source} = M/(1+z)$.
\end{itemize}

==> zz-imp/back-imp-cv.tex <==
\chapter{Curriculum Vitae}
\vspace{\parskip}
\begingroup
\renewcommand*{\arraystretch}{1.5}
\begin{tabular}{@{} >{\bfseries}p{0.45\textwidth}  p{0.52\textwidth} @{}}
\MakeUppercase{Name}          & \asserttoken{dissertationAuthorName}{Firstname Lastname} \\
\addlinespace[4ex]

\MakeUppercase{Date of Birth} & \asserttoken{dissertationDateOfBirth}{01 January 2022}   \\
\addlinespace[4ex]
%
%
%
\MakeUppercase{Education Qualifications} &
\end{tabular}

\input 3-backmatter/back-cv-education
\endgroup


==> zz-imp/pre-imp-cert.tex <==
\chapter*{Thesis Certificate}
This is to undertake that the \asserttoken{dissertationType}{Whatever} titled
%{\bfseries\MakeUppercase{\asserttoken{dissertationTitle}{Whatever Title}}},
{\bfseries{Synergies in analysing binary black hole
mergers: Effect of orbital eccentricity, spin-precession, and non-quadrupole modes}},
submitted by me to the Indian Institute of Technology Madras, for the award of
{\bfseries\asserttoken{dissertationDegree}{Whatever Degree}}, is a bona fide
record of the research work done by me under the supervision of
{\bfseries\asserttoken{dissertationGuides}{Whoever Guides}}. The contents of
this \asserttoken{dissertationType}{Whatever}, in full or in parts, have not
been submitted to any other Institute or University for the award of any degree
or diploma.
\par

\IfFileExists{0-prematter/pre-cert-attr.tex}
    {\input 0-prematter/pre-cert-attr
    }
    {}
\vspace{3\parskip}

\hfill \includegraphics[trim=0 5 15 10, clip, width=0.25\linewidth]{images/Divyajyoti - Signature.jpg}
\vspace{-1em}

\begin{tabular}{@{} >{\bfseries}p{0.48\textwidth} >{\bfseries\raggedleft}p{0.48\textwidth} @{}}
\begin{tabular}[t]{@{} p{0.48\textwidth} @{}}
Chennai 600036 \newline
Date:  {\bfseries
        \asserttoken{dissertationCertificateDate}
          {01 January 2022}}
\end{tabular}
    &
\asserttoken{dissertationAuthorName}{Firstname Lastname} \tabularnewline
\end{tabular}
\input 0-prematter/pre-cert-guides
\vspace*{\fill}
\textcopyright\ \asserttoken{dissertationYear}{2022}\ Indian Institute of Technology Madras
\newpage

